Algebraic $k$-sets and generally neighborly embeddings

Given a set $S$ of $n$ points in $\mathbb{R}^d$, a $k$-set is a subset of $k$ points of $S$ that can be strictly separated by a hyperplane from the remaining $n-k$ points. Similarly, one may consider $k$-facets, which are hyperplanes that pass through $d$ points of $S$ and have $k$ points on one side. A notorious open problem is to determine the asymptotics of the maximum number of $k$-sets. In this paper we study a variation on the $k$-set/$k$-facet problem with hyperplanes replaced by algebraic surfaces. In stark contrast to the original $k$-set/$k$-facet problem, there are some natural families of algebraic curves for which the number of $k$-facets can be counted exactly. For example, we show that the number of halving conic sections for any set of $2n+5$ points in general position in the plane is $2\binom{n+2}{2}^2$. To understand the limits of our argument we study a class of maps we call \emph{generally neighborly embeddings}, which map generic point sets into neighborly position. Additionally, we give a simple argument which improves the best known bound on the number of $k$-sets/$k$-facets for point sets in convex position.

==> article.tex <==
\def\overrideversion{\defaultversion}
\input{main.tex} 

==> bad.tex <==

\begin{prop}
Assume that there is a set of $n$ points in $\Rl^2$ with at least $nf(k)$ $\lceil k/2 \rceil$-edges. Then there exists a set of $n$ points in $\Rl^2$ with $\Omega(nkf(k))$ $\F_{Hyp}$-$k$-sets. 
\end{prop}
\begin{proofidea}
We explain the idea for the ``halving case.''
Let $S'$ be a set of $n/2$ points in $\RR^2$ with $\Omega(nf(n))$ halving edges.
By applying a suitable affine transformation, we can assume that all lines spanned by $S'$ are very close to a fixed line $l$ that passes through the origin.
Identify $\RR^2$ with the $xy$-plane in $\RR^3$ and embed $S'$ in that way.
Let $V \subseteq \RR^2$ be a configuration of $n/2$ points so that every line through the origin and a point in $V$ is a halving line ($V$ is the set of vertices of an regular $(n/2)-gon$ for odd $n/2$).
Embed $\RR^2 \supseteq V$ as the orthogonal complement of $l$ in $\RR^3$.
Then for any halving edge $pq$ in $S'$ we have $n/2$ halving triangles $pqr$ for $r \in V$.
The challenge now is to move all points to the embedded manifold while preserving the number of halving triangles.
It would be natural to embed $S'$ so that $l$ embeds into the $x$ axis (the $x$ axis lies on the embedded manifold), but it is not clear how to make the point movement small enough.
Instead, we will rotate the manifold $45^\circ$ on the $xy$-plane and embed $l$ still into the $x$ axis. 
The rotated manifold is the result of the embedding $(x,y) \mapsto (x,y,x^2-y^2)$ (up to scaling).
If we consider the embedding for $y=0$, we see that the manifold contains the parabola $(x,0) \mapsto (x,0,x^2)$, tangent to $l$.
The quadratic behavior of the parabola near the origin provides better control of the point movement.
\end{proofidea}


\begin{proof}
Let $H'$ consist of $n-2\lfloor k/2 \rfloor-1$ points in the plane with $\Omega(nf(k))$ $\lceil k/2\rceil$-edges. 

\end{proof}





\begin{proof} 
Since $V$ has real dimension $n$, the dimension of $V$ as an algebraic variety must be at least $n$. Let $L$ be a $(d-n+1)$-flat meeting $\interior(\conv(V))$\lnote{why is int nonempty?} and passing through some smooth point $p$ of $V$. 
By Theorem 12 in \cite{Seidenberg1950TheHS}, $L$ can be perturbed slightly so that $L \cap V$ is irreducible and 1-dimensional. Furthermore, by Bertini's theorem (for example Theorem 9.6.4 in \cite{Bochnak}), $L$ can be perturbed so that $L \cap V$ has no singular points other than perhaps singular points of $V$. In particular, we can assume that $p$ is a smooth point of $L \cap V$. Since $L\cap V$ contains a smooth point, by 2.8.14 in \cite{Bochnak}, the real dimension of $L \cap V$ is 1. 

With these guarantees, we claim that one can find arbitrarily large $k$-neighborly point sets contained in $L \cap V$. Let $S$ be a $k$-neighborly set of $m$ points on $L \cap V$. Since $V$ is generally $k$-neighborly, by Lemma 2\lnote{xxx}, for each $I \in  \binom{S}{k}$, there exists a hyperplane $H_I \subset \RR^d$ such that $I \subset H_I$ and $V \subset H_I^+$. Note that there may not be a unique hyperplane $H_I$ with this property. In what follows, assume that for each $I$ we have chosen a specific hyperplane $H_I$ such that $I \subset H_I$ and $V \subset H_I^+$. 

Before proceeding, we need to add an additional assumption on the point set $S$. Recall that we have assumed that $S$ is $k$-neighborly and so for each $I \in \binom{S}{k}$, the points in $I$ form a face of the convex hull of $S$. However, for some $I$ it may not be the case that $H_I$ supports the face formed by $I$. This could happen if perhaps $H_I$ contained some points of $S \setminus I$. We need to assume that $S$ is a $k$-neighborly set of $m$ points on $L \cap V$. And we need to assume further that the hyperplanes $H_I$ actually support the face formed by the points of $I$. 

In summary, we are assuming that $S$ is a set of $m$ points on $L \cap V$ and that for each $I \in \binom{S}{k}$ there exists a hyperplane $H_I$ such that $I \subset H_I$, $V \subset H_I^+$ and $(S \setminus I) \cap H_I = \emptyset$. Again, the hyperplanes $H_I$ satisfying the above conditions may not be unique. Assume that for each $I$ we have fixed some $H_I$ that has these conditions. 

We will now use $S$ to show that there exists a set $S'$ of $m+1$ points on $L \cap V$ with precisely the same properties summarized in the previous paragraph. By induction it will then follow that there exists arbitrarily large point sets on $L \cap V$ with these properties and thus it follows that there exists arbitrarily large $k$-neighborly point sets on $L \cap V$. 

First we need to choose some $s$ that is not contained in any of the supporting hyperplanes $\{H_I: I \in \binom{S}{k}\}$. That is, we need to choose some $s$ not contained in 
\[
B := L \cap V \cap \bigg(\bigcup_{I \in \binom{S}{k}}H_I\bigg).
\]
To show that such an $s$ always exists, we need to verify that $L \cap V \not\subset B$. First note that each hyperplane $H_I$ does not intersect $\interior(\conv(V))$. 
This shows that $L \cap V$ is not contained in any one $H_I$. Also, it shows that for each $I$, $H_I\cap L$ is a proper hyperplane in $L$. Now, if it were the case that $L\cap V \subset B$ we would have a decomposition
\[
L \cap V = \bigcup_{I \in \binom{S}{k}} (L \cap V \cap H_I).
\]
Since we already know that $L \cap V$ is not contained in any one $H_I$, this would be a representation of $L \cap V$ as the union of proper closed subvarieties. This is impossible since $L\cap V$ is irreducible. Therefore we know that $L \cap V  \not\subset B$. 

Choose some $s \in L \cap V \setminus B$. We have immediately that for each $I \in \binom{S}{k}$, the points of $I$ form a face of $\conv(S \cup \{s\})$\lnote{probably true but not convinced. the hyperplane that proves k-neighborly is not necessarily $H_I$. What if $s$ is outside? Maybe fixable with the invariant: points $S$ together with planes $H_I$ that prove $k$-neighborliness and weakly.}. \bnote{I think this has now been fixed (10/29)}
However, it could be that for some $J \in \binom{S}{k-1}$, $H_{J \cup \{s\}}$ contains some point of $S \setminus J$, in which case $J \cup \{s\}$ would not necessarily form a face of $\conv(S \cup \{s\})$. In order to fix this issue, the points of $S$ need to be perturbed slightly along $L \cap V$. 


Observe that for each $v \in S$, there exists a ball $B_v$ containg $v$ such that moving $v$ within $B_v$ does not change the facial structure of $\conv(S)$. 

First of all, this allows us to assume that all points of $S$ are smooth points of $V \cap L$. Indeed, since the smooth points of a variety are dense, if $S$ contains any singular points, those points can be perturbed slightly to smooth points. 

Now, if it is the case that $v \in H_{ J \cup \{s\}}$ for some $J \in \binom{S}{k-1}$ and $v \in S \setminus J$, $v$ can be perturbed within $B_v$ so that this is no longer the case. The reason why this is true is that no hyperplane in $L$ can contain any open neighborhood of $v$ in $L \cap V$. This is due to the following fact: 

Fact: Let $X$ be an irreducible real algebraic variety and let $x$ be a smooth point of $X$. If $f$ is a polynomial which vanishes on a neighborhood of $x$ in $X$, then $X \subset V(f)$. 

Applied to our situation, if $H$ was a hyperplane containing a neighborhood of $v$, the fact implies that $H$ contains $L \cap V$. But this is impossible since $H$ supports $V$ and $L$ intersects the interior of $\conv(V)$. \lnote{is H any of the $H_I$ or something else? Also containment in fact and use seems reversed.}. 

After performing all necessary perturbations, we have that $S \cup \{s\}$ is a neighborly configuration of $m+1$ points on $L \cap V$. 

This argument can be repeated and so we can add any finite number of points to $L \cap V$ while maintaining $k$-neighborliness of the point set. Recall that a $k$-neighborly polytope which is not a simplex cannot exist in less than $2k$ dimensions. Therefore, since we can find $d+2$ points on $L \cap V$ which are the vertices of a $k$-neighborly polytope we have shown that $d-n+1 \ge 2k$. 

\end{proof}




Assume not, so that there exists $T \subset M$ with $|T| = k$ such that every hyperplane $H$ containing $T$ is such that there is some $s_1,s_2$ such that  $s_1 \in (H^+ \setminus H)\cap M$ and $s_2 \in (H^- \setminus H) \cap M$. We want to argue that if this were the case then the general position assumption for $\varphi$ would have to remove a subset of point configurations with nonempty interior. Indeed, assuming we are in the situation as above, we could find small balls $\{B_t  : t \in T\}$ centered at the points of $T$ and small balls $B_{s_1},B_{s_2}$ centered at $s_1,s_2$ such that any configuration of points with one point from each of the balls $B_{s_1},B_{s_2}$ and each $B_t$ would not be neighborly. Therefore, the general position assumption would have to remove all point configurations in $B_{s_1} \times B_{s_2} \times B_{t_1} \times \dotsc \times B_{t_k} \subset \Rl^{n(k+2)}$ which has nonempty interior. 


\begin{lemma}
If $\varphi: \Rl^n \to \Rl^d$ is a generally $k$-neighborly embedding (or polynomial map) with general position assumption $G$, then any finite subset of $M:=\varphi(\Rl^n)$ is weakly $k$-neighborly. 
\end{lemma}
\begin{proof}
Assume not, so that there exists some finite set $S \subset M$  and a set $T$ of $k$ points from $S$ such that no halfspace contains $S$ and contains $T$ on its boundary. This means that $\conv(T)$ intersects the interior of $\conv(S \setminus T)$. We can find small balls $\{B_i: i \in S\}$ such that any configuration of points consisting of one point from each ball is not $k$-neighborly. This means that no configuration $C \subset \Rl^{n|S|}$ of $|S|$ points consisting of one point from each ball satisfies the general position assumption $G$. Observe that the product of balls has non-empty interior. Therefore the set configurations of size $|S|$ which do not satisfy the general position assumption has non empty interior in $\Rl^{n|S|}$, a contradiction to Definition 1. 
\end{proof}




\begin{lemma}
If $\varphi: \Rl^n \to \Rl^d$ is a generally $k$-neighborly embedding with general position assumption $G$, then $M:=\varphi(\Rl^n)$ is weakly $k$-neighborly. 
\end{lemma}


\begin{proof}
Assume not, so that there exists set $T = \{v_1, \dotsc , v_k \}$ of $k$ points from on $M$ such that no halfspace contains $M$ and contains $T$ on its boundary. This means that $\relint(\conv(T)) \cap \relint(\conv(M)) \neq \emptyset$ (cite http://page.mi.fu-berlin.de/sanyal/teaching/dg2/DG2-Skript.pdf) Therefore, by Caratheodory? there exists a finite set $S \subset M$ such that $\relint(\conv(T)) \cap \relint(\conv(S)) \neq \emptyset$. By adding points if necessary we can assume that $\aff(S,T) = \Rl^d$. 

We can find balls $\{B_i : 1 \le i \le k\}$ and $\{A_j: j \in S\}$ such that $v_i \in B_i$ $s_j \in B_j$ and given any choice of points $T' = \{v_1', \dotsc, v_k' : v_i' \in B_i\}$, and $S' =\{s_1', \dotsc, s_{|S|}' : s_j' \in A_j\}$ we have that  $\relint(\conv(T')) \cap \relint(\conv(S')) \neq \emptyset$. By Lemma 32, this implies that $S'$ and $T'$ cannot be weakly separated and so $T'$ cannot be a face of $\conv(S,T)$. This means that the set of point configurations of size $k+|S|$ violating $G$ would have to contain $B:=\varphi^{-1}(B_1 \times \dotsc \times B_k \times A_1 \times \dotsc \times A_{|S|})$. Observe that since each ball $B_i$ contains a point of $M$, it contains a neighborhood homeomorphic to $\Rl^n$. Therefore, $B$ has nonempty interior in $\Rl^{n(|S|+k)}$, a contradiction. 
\end{proof}


==> oldgeneralposition.tex <==
\section{General position}
After defining $k$-sets and $k$-facets for set systems other than halfspaces, we will need to use various general position assumptions different from general linear position. 

In \cref{sec:generally}, we study the minimal possible $p$ among maps $\varphi:\RR^d \to \RR^p$ that embed generic point sets into $k$-neighborly point sets.
So, we need a precise criterion for deciding what is an acceptable notion of general position for point sets. 
This criterion is described below.
See \cite[Section 1.1]{Matousek} for more on general position. 
Our lower bound on $p$ works with a criterion that allows notions of general position that have very few generic point sets, and this makes the bound stronger.
Namely, even maps that embed very few point sets into a $k$-neighborly point set are proven to be impossible.

At the same time, our upper bound and other explicit constructions of maps, have general position assumptions that are more standard and have many generic point sets.
In particular, they are of the kind described in the next paragraph (zero set of some multivariate polynomial).

A crucial property of general position for point sets in $\Rl^d$ is that any configuration of points has some configuration in general position arbitrarily close to it. 
One way of guaranteeing this is by describing the point sets which violate the general position assumption by the zero set of some multivariate polynomial: 
Say we have an $n$-point set $S$ in $\Rl^d$. 
The collection of all configurations of $n$-point sets in $\Rl^d$ can be identified with $\Rl^{dn}$. 
In this case, the general position assumption put on $S$ is that $P(t_1, \dotsc ,t_{dn}) \neq 0$ for some nonzero polynomial $P$ in $dn$ variables. 
In this setup, say $N \subset \Rl^{dn}$ is the collection of point configurations which do not satisfy the general position assumption. 
Then it is always the case that $N$ has empty interior in $\Rl^{dn}$. 
This further motivates our definition of general position.

\begin{definition}\label{def:generalposition}
A \emph{general position assumption} for point sets in $\Rl^d$ is any condition on point sets in $\Rl^d$ that has the property that for each $n \in \Nl$, the set of configurations $N \subset \Rl^{dn}$ which do not satisfy the condition has empty interior in $\Rl^{dn}$\details{iff complement is dense}.
\end{definition}
\lnote{maybe explain how it is used later?}
%Note: This definition is in a sense as unrestrictive as possible. Recall that it is a crucial property of general position assumptions on point sets that any configuration of points must have some configuration in general position arbitrarily close to it. 
%This property is equivalent to the property that the set $N$ of configurations violating the general position assumption has empty interior. 






Essentially the same proof shows the corresponding result for generally $k$-neighborly varieties:
\begin{lemma}\label{lem:polyweakly}
If $V$ is a generally $k$-neighborly algebraic variety, then every finite set of points on $V_{\text{sm}}$ is weakly $k$-neighborly.
\end{lemma}
\makeproof{}{lem:polyweakly}{
%\begin{proof}
The proof of \cref{lem:generallyweakly} holds with one change. 
We need to argue why $B_1 \times \dotsb \times B_k\times A_1 \times \dotsb \times A_{|S\setminus T|}$ contains a subset homeomorphic to $\Rl^{d|S|}$. 
This is because each $A_i, B_i$ contains a smooth point of $V$ and so contains a neighborhood of that smooth point which is homeomorphic to $\Rl^d$. And so the previous argument also works in this case. 
%\end{proof}
}


==> oldproof.tex <==
\lnote{recall used too many times in proof}
\makeproof{}{thm:lowerboundweak}{
%\begin{proof}[Proof of \cref{thm:lowerboundweak}]

First we will show that we can find a flat $L$ of an appropriate dimension that intersects the interior of the convex hull of $V_{\text{sm}}$ and such that $L$ intersects $V$ in a non-degenerate irreducible real algebraic variety of dimension at least 1.

In order to find such a flat $L$ we need to establish the following claim: Assume that $V \subset \Rl^p$ is an irreducible $d$-dimensional ($d \ge 2$) non-degenerate variety with a smooth real point. Assume also that $V_{sm}$ is weakly $k$-neighborly but not weakly $(k+1)$-neighborly and that $p \ge k+1$. Then there exists hyperplane $H$ such that $H$ intersects $\interior \conv V_{sm}$ and $V \cap H$ is an irreducible, non-degenerate, $(d-1)$-dimensional variety with a smooth real point. 

We want to start by finding a hyperplane $H$ which intersects $\interior(\conv(V_{\text{sm}}))$ and such that $H$ is spanned by smooth points of $V$. 

Since $V_{sm}$ is not weakly $(k+1)$-neighborly, there exists a set $T$ of $k+1$ points from $V_{\text{sm}}$ such that no closed halfspace contains $V_{\text{sm}}$ and contains $T$ on its boundary. By the separating hyperplane theorem \cite[Theorem 1.3.8]{MR3155183}, $\aff(T) \cap \relint \conv(V_{\text{sm}} \setminus T) \neq \emptyset$. Observe that the points of $T$ are affinely independent since if not then there would be a subset $R \subset T$ of size at most $k$ such that $\aff(R) \cap \relint \conv(V_{\text{sm}}) \neq \emptyset$, a contradiction to weakly $k$-neighborliness of $V_{\text{sm}}$. Choose $p-k-1$ additional points $u_1, \dotsc , u_{p-k-1}$ on $V_{\text{sm}}$ so that $U:= T\cup \{u_1, \dotsc, u_{p-k-1}\}$ is affinely independent. This can always be done because $V_{\text{sm}}$ is non-degenerate by \cref{prop:smoothnd}. 
Now letting $H = \aff(U)$, $H$ is a hyperplane with the properties outlined at the beginning of the paragraph. Indeed, since $\aff(T) \cap \relint \conv(V_{\text{sm}} \setminus T) \neq \emptyset$, we know that $H \cap \interior \conv V_{\text{sm}} \neq \emptyset$. And since $H$ is spanned by $p$ affinely independent points on $V_{\text{sm}}$, we know that $H \cap V$ is nondegenerate in $H$. 

Now we will find a new hyperplane $H'$ close to $H$ which has the additional properties that $H' \cap V$ is irreducible and contains a smooth real point. And we will maintain that $H'$ intersects $\interior \conv V_{sm}$ and that $H' \cap V$ is non-degenerate. 

Let $\mathcal{H}$ be the set of hyperplanes in $\Rl^p$. We identify $\mathcal{H}$ with $\mathbb{P}^p(\Rl)$. Let $I \subset \mathcal{H}$ be the set of hyperplanes $H$ such that $(H \cap V)_{\Cx}$ is irreducible and at least $(d-1)$-dimensional. By \cite[Theorem 12]{Seidenberg1950TheHS}, $I^c$ is a proper closed (projective) subvariety of $\mathcal{H}$. For our purposes, we only need to know that $I^c$ is closed with empty interior, i.e., $I$ is open and dense. The condition that $(H \cap V)_{\Cx}$ is irreducible also guarantees that $H \cap V$ is irreducible, see \cref{sec:alggeo}.

Let $O \subset \mathcal{H}$ be the set of hyperplanes which intersect $\interior(\conv(V_{sm}))$. The set $O$ is open and contains $H$. 

For each $u \in U$, let $B_u \subset \RR^p$ be a ball centered at $u$. The radii of the balls can be chosen small enough so that any configuration of points consisting of one point from each $B_u$ is non-degenerate and so that any hyperplane spanned by a set of points consisting of one point from each $B_u$ is in $O$. Let $A_u = \{x \in \Rl^p : x \in \aff((U \setminus u) \cup v) \cap B_u \text{ for some $v \in V_{sm} \cap B_u$ }\}$. Since $V$ is an irreducible variety, by \cref{prop:smoothnbhd}, $V \cap B_u$ is not contained in $H$. Therefore, the set of hyperplanes spanned by point sets consisting of one point from each $A_u$ has non-empty interior. Therefore, letting $N \subset O$ be the set of hyperplanes $H$ such that $H\cap V_{sm}$ is non-degnerate, we have that $N$ has nonempty interior in $O$. 

Let $S \subset \mathcal{H}$ be the set of hyperplanes $H$ for which $H \cap V$ has no singular points other than perhaps singular points of $V$. Then we claim that $S$ is open and dense in $\mathcal{H}$. This follows from Bertini's theorem \cite[Theorem 17.16]{Harris}. First consider the complex variety $V_{\Cx}$. Let $S' \subset \mathbb{P}^p(\Cx)$ be the set of complex hyperplanes $H$ such that $H \cap V_{\Cx}$ has no singular points other than perhaps singular points of $V$. Applying Bertini's theorem as in \cite{Harris} shows that $S'$ is open and dense. Therefore, $S \subset \mathcal{H}$ is also open. Because $\mathcal{H}$ is dense in $\mathbb{P}^p(\Cx)$ (in the Zariski topology), we get that $S$ is dense as well.

%By Bertini's Theorem (Theorem 9.6.4 in \cite{Bochnak}), $S$ is open and dense. 

This means that $N \cap O \cap I \cap S \neq \emptyset$. Indeed, because $I$ and $S$ are open and dense, $I \cap S$ is open and dense. Therefore, since $N \cap O$ has non-empty interior $N \cap O$ is not contained in $I^c \cup S^c$. Any $H \in N \cap O \cap I\cap S$ satisfies the requirements of the claim. 

Now set $m = \max(p-n+1,k)$. We can assume without loss of generality that the variety $V$ in the statement of the theorem is $k$-neighborly but not $(k+1)$-neighborly. By taking succesive hyperplane sections, we can find an $m$-flat $L$ such that $C:=L \cap V$ is a non-degenerate irreducible variety of dimension at least 1 with a smooth real point. 

Now we will show that one can find arbitrarily large point sets in general linear position on $C \cap V_{\text{sm}}$. In order to accomplish this we first show that $C \cap V_{\text{sm}}$ is non-degenerate. Indeed, if it were the case that $C \cap V_{sm}$ has contained in a hyperplane $H$, then we would have $C = (C \cap H) \cup (C \cap V_{\text{sing}})$ which is impossible since $C$ is irreducible. 

Now assume that $S$ is a set of $j$ points in general linear position on $C \cap V_{\text{sm}} $. If it were not possible to find another point $s$ such that $S \cup  \{s\}$ is in general linear position, it would have to be the case that $C \cap V_{\text{sm}}$ is contained in the union of all hyperplanes in $L$ spanned by $p$ points from the set $S$. Let $\mathcal{H}$ be the collection of all hyperplanes in $L$ spanned by $p$ points in $S$. Note that $\mathcal{H}$ is finite. We have
\[
C = (C \cap V_{\text{sm}}) \cup ( C\cap V_{\text{sing}})= \bigg(\bigcup_{H \in \mathcal{H}} (C \cap V_{sm} \cap H) \bigg) \cup (C \cap V_{\text{sing}}).
\]
Since $C \cap V_{sm} $ is non-degenerate the above formula would be a representation of $C$ as the union of proper subvarieties. This is impossible since $C$ is irreducible. Therefore we know that $C \cap V_{\text{sm}}$ is not contained in the union of all hyperplanes in $L$ spanned by points in $S$ and so we can always find $s$ so that $S \cup \{s\}$ is in general linear position. It follows that we can find arbitrarily large point sets in general linear position on $C \cap V_{\text{sm}}$.








Let $P$ be a set of $m+2$ points in general linear position on $C \cap V_{sm}$. By \cref{lem:radon,lem:separation}, there is a partition $Q,R$ of $P$ into non-empty sets so that $Q,R$ cannot be weakly separated (in $L$). 

However, because $V_{\text{sm}}$ is weakly $k$-neighborly, we know that for any set $T$ of $k$ points on $C\cap V_{sm}$ there exists a closed halfspace $H$ (in $\Rl^p$) which contains $V_{\text{sm}}$ and contains $T$ in $\bd(H)$. 
In other words, any such $T$ can be weakly separated from $V_{\text{sm}}$. 
Notice that we are talking about weak separation in $\Rl^p$, while we are really interested in weak separation in $L$. 
We claim that our assumption that $L$ intersects the interior of the convex hull of $V_{\text{sm}}$ allows us to pass from weakly separating hyperplanes in $\Rl^p$ to weakly separating hyperplanes in $L$. 
Indeed, the fact that $L$ intersects $\interior(\conv(V_{\text{sm}}))$ means that any closed halfspace $H$ satisfying $V_{\text{sm}} \subset H$  cannot contain $L$ in its boundary. 
Therefore $\bd(H) \cap L$ is a proper hyperplane in $L$. 
To summarize, given a set $T$ of $k$ points on $C\cap V_{sm}$, by the assumption that any finite set on $V_{sm}$ is weakly $k$-neighborly, there exists a hyperplane $\bd(H)$ that weakly separates $T$ from $V_{sm}$. 
This and the way we chose $L$ allows us to conclude that $\bd(H) \cap L$ is a hyperplane in $L$ that weakly separates $T$ from $C\cap V_{sm}$.

Therefore, we have that any set of $k$ points on $C\cap V_{sm}$ can be weakly separated (in $L$) from any other finite set of points on $C \cap V_{sm}$. However, recall that we found a set $P$ of $m+2$ points on $C \cap V_{sm}$  such that  there is a partition $Q,R$ of $P$ into non-empty sets so that $Q,R$ cannot be weakly separated (in $L$).  Now since $\min(|Q|,|R|)  \le \lfloor\frac{m+2}{2}\rfloor$, we have that $k \le \lfloor\frac{m+2}{2}\rfloor - 1$. If $m = k$, then we get $k \le \lfloor\frac{k+1}{2}\rfloor - 1$ which implies $k \le 0$ in which case $p \ge 2k+d-1$ is immediate. If $m = p-d+1$ we get $k \le \lfloor\frac{p-d+3}{2}\rfloor - 1$ and so $p \ge 2k+d-1$.
%\end{proof}
}




Finally we establish two basic facts about varieties which will be used later.

\begin{proposition}\label{prop:smoothnd}
If $V$ is a non-degenerate irreducible variety with a smooth real point, then $V_{sm}$ is non-degenerate. 
\end{proposition}
\begin{proof}
Recall that the set of singular points of a real variety forms a proper closed subvariety \cite[Theorem 4.8]{Sheffer}. Therefore, if it was the case that $V_{\text{sm}}$ is contained in some hyperplane $H$, then $(H\cap V) \cup V_{\text{sing}}$ would be a decomposition of $V$ as the union of proper closed subvarieties which is impossible since $V$ is irreducible.
\end{proof}


\begin{proposition}\label{prop:smoothnbhd}
If $V$ is a non-degenerate $d$-dimensional irreducible variety and $u$ a smooth point of $V$, no open neighborhood of $u$ in $V$ is contained in a hyperplane.
\end{proposition}
\begin{proof}
Assume $U \subset V$ is some open neighborhood of $u$ contained in a hyperplane $H$. Then we have that the real dimension of $H \cap V$ is equal to $d$ which implies that the dimension of $H \cap V$ as a variety is at least $d$. Therefore, there is chain $V_{0}\subsetneq V_{1}\subsetneq \ldots \subsetneq V_{d-1} \subsetneq V_d$  of length $d$ of non-empty irreducible subvarieties of $V \cap H$. Since $V$ is non-degenerate, $V_d \subset V \cap H \subsetneq V$. So there is a chain $V_{0}\subsetneq V_{1}\subsetneq \ldots \subsetneq V_{d-1} \subsetneq V_d \subsetneq V$ of non-empty irreducible subvarieties of $V$ which implies that the dimension of $V$ is at least $d+1$, a contradiction. 
\end{proof}




Let $I \subset \mathbb{P}^p(\Rl)$ be the set of hyperplanes $H$ such that $(H \cap V)_{\Cx}$ is irreducible and at least $(d-1)$-dimensional. By \cite[Theorem 12]{Seidenberg1950TheHS}, $I^c$ is a proper closed (projective) subvariety of $\mathbb{P}^p(\Rl)$. Therefore, $I$ is open and dense.

==> oursvjour3thm.tex <==
% definition of the "\spnewtheorem" command.
%
% Usage:
%
%     \spnewtheorem{env_nam}{caption}[within]{cap_font}{body_font}
% or  \spnewtheorem{env_nam}[numbered_like]{caption}{cap_font}{body_font}
% or  \spnewtheorem*{env_nam}{caption}{cap_font}{body_font}
%
% New is "cap_font" and "body_font". It stands for
% fontdefinition of the caption and the text itself.
%
% "\spnewtheorem*" gives a theorem without number.
%
% A defined spnewthoerem environment is used as described
% by Lamport.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\@thmcountersep{}
\def\@thmcounterend{}
\newcommand\nocaption{\noexpand\@gobble}
\newdimen\spthmsep \spthmsep=5pt

\def\spnewtheorem{\@ifstar{\@sthm}{\@Sthm}}

% definition of \spnewtheorem with number

\def\@spnthm#1#2{%
  \@ifnextchar[{\@spxnthm{#1}{#2}}{\@spynthm{#1}{#2}}}
\def\@Sthm#1{\@ifnextchar[{\@spothm{#1}}{\@spnthm{#1}}}

\def\@spxnthm#1#2[#3]#4#5{\expandafter\@ifdefinable\csname #1\endcsname
   {\@definecounter{#1}\@addtoreset{#1}{#3}%
   \expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
     \csname the#3\endcsname \noexpand\@thmcountersep \@thmcounter{#1}}%
   \expandafter\xdef\csname #1name\endcsname{#2}%
   \global\@namedef{#1}{\@spthm{#1}{\csname #1name\endcsname}{#4}{#5}}%
                              \global\@namedef{end#1}{\@endtheorem}}}

\def\@spynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
   {\@definecounter{#1}%
   \expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
   \expandafter\xdef\csname #1name\endcsname{#2}%
   \global\@namedef{#1}{\@spthm{#1}{\csname #1name\endcsname}{#3}{#4}}%
                               \global\@namedef{end#1}{\@endtheorem}}}

\def\@spothm#1[#2]#3#4#5{%
  \@ifundefined{c@#2}{\@latexerr{No theorem environment `#2' defined}\@eha}%
  {\expandafter\@ifdefinable\csname #1\endcsname
  {\global\@namedef{the#1}{\@nameuse{the#2}}%
  \expandafter\xdef\csname #1name\endcsname{#3}%
  \global\@namedef{#1}{\@spthm{#2}{\csname #1name\endcsname}{#4}{#5}}%
  \global\@namedef{end#1}{\@endtheorem}}}}

\def\@spthm#1#2#3#4{\topsep 7\p@ \@plus2\p@ \@minus4\p@
\labelsep=\spthmsep\refstepcounter{#1}%
\@ifnextchar[{\@spythm{#1}{#2}{#3}{#4}}{\@spxthm{#1}{#2}{#3}{#4}}}

\def\@spxthm#1#2#3#4{\@spbegintheorem{#2}{\csname the#1\endcsname}{#3}{#4}%
                    \ignorespaces}

\def\@spythm#1#2#3#4[#5]{\@spopargbegintheorem{#2}{\csname
       the#1\endcsname}{#5}{#3}{#4}\ignorespaces}

\def\normalthmheadings{\def\@spbegintheorem##1##2##3##4{\trivlist\normalfont
                 \item[\hskip\labelsep{##3##1\ ##2\@thmcounterend}]##4}
\def\@spopargbegintheorem##1##2##3##4##5{\trivlist
      \item[\hskip\labelsep{##4##1\ ##2}]{##4(##3)\@thmcounterend\ }##5}}
\normalthmheadings

\def\reversethmheadings{\def\@spbegintheorem##1##2##3##4{\trivlist\normalfont
                 \item[\hskip\labelsep{##3##2\ ##1\@thmcounterend}]##4}
\def\@spopargbegintheorem##1##2##3##4##5{\trivlist
      \item[\hskip\labelsep{##4##2\ ##1}]{##4(##3)\@thmcounterend\ }##5}}

% definition of \spnewtheorem* without number

\def\@sthm#1#2{\@Ynthm{#1}{#2}}

\def\@Ynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
   {\global\@namedef{#1}{\@Thm{\csname #1name\endcsname}{#3}{#4}}%
    \expandafter\xdef\csname #1name\endcsname{#2}%
    \global\@namedef{end#1}{\@endtheorem}}}

\def\@Thm#1#2#3{\topsep 7\p@ \@plus2\p@ \@minus4\p@
\@ifnextchar[{\@Ythm{#1}{#2}{#3}}{\@Xthm{#1}{#2}{#3}}}

\def\@Xthm#1#2#3{\@Begintheorem{#1}{#2}{#3}\ignorespaces}

\def\@Ythm#1#2#3[#4]{\@Opargbegintheorem{#1}
       {#4}{#2}{#3}\ignorespaces}

\def\@Begintheorem#1#2#3{#3\trivlist
                           \item[\hskip\labelsep{#2#1\@thmcounterend}]}

\def\@Opargbegintheorem#1#2#3#4{#4\trivlist
      \item[\hskip\labelsep{#3#1}]{#3(#2)\@thmcounterend\ }}

% initialize theorem environment

\if@envcntsect
   \def\@thmcountersep{.}
   \spnewtheorem{theorem}{Theorem}[section]{\bfseries}{\itshape}
\else
   \spnewtheorem{theorem}{Theorem}{\bfseries}{\itshape}
   \if@envcntreset
      \@addtoreset{theorem}{section}
   \else
      \@addtoreset{theorem}{chapter}
   \fi
\fi

%definition of divers theorem environments
\spnewtheorem*{claim}{Claim}{\itshape}{\rmfamily}
%\spnewtheorem*{proof}{Proof}{\itshape}{\rmfamily}
\if@envcntsame % all environments like "Theorem" - using its counter
   \def\spn@wtheorem#1#2#3#4{\@spothm{#1}[theorem]{#2}{#3}{#4}}
\else % all environments with their own counter
   \if@envcntsect % show section counter
      \def\spn@wtheorem#1#2#3#4{\@spxnthm{#1}{#2}[section]{#3}{#4}}
   \else % not numbered with section
      \if@envcntreset
         \def\spn@wtheorem#1#2#3#4{\@spynthm{#1}{#2}{#3}{#4}
                                   \@addtoreset{#1}{section}}
      \else
         \let\spn@wtheorem=\@spynthm
      \fi
   \fi
\fi
%
\let\spdefaulttheorem=\spn@wtheorem
%
\spn@wtheorem{case}{Case}{\itshape}{\rmfamily}
\spn@wtheorem{conjecture}{Conjecture}{\itshape}{\rmfamily}
\spn@wtheorem{corollary}{Corollary}{\bfseries}{\itshape}
\spn@wtheorem{definition}{Definition}{\bfseries}{\rmfamily}
\spn@wtheorem{example}{Example}{\itshape}{\rmfamily}
\spn@wtheorem{exercise}{Exercise}{\bfseries}{\rmfamily}
\spn@wtheorem{lemma}{Lemma}{\bfseries}{\itshape}
\spn@wtheorem{note}{Note}{\itshape}{\rmfamily}
\spn@wtheorem{problem}{Problem}{\bfseries}{\rmfamily}
\spn@wtheorem{property}{Property}{\itshape}{\rmfamily}
\spn@wtheorem{proposition}{Proposition}{\bfseries}{\itshape}
\spn@wtheorem{question}{Question}{\itshape}{\rmfamily}
\spn@wtheorem{solution}{Solution}{\bfseries}{\rmfamily}
\spn@wtheorem{remark}{Remark}{\itshape}{\rmfamily}
%
\newenvironment{theopargself}
    {\def\@spopargbegintheorem##1##2##3##4##5{\trivlist
         \item[\hskip\labelsep{##4##1\ ##2}]{##4##3\@thmcounterend\ }##5}
     \def\@Opargbegintheorem##1##2##3##4{##4\trivlist
         \item[\hskip\labelsep{##3##1}]{##3##2\@thmcounterend\ }}}{}
\newenvironment{theopargself*}
    {\def\@spopargbegintheorem##1##2##3##4##5{\trivlist
         \item[\hskip\labelsep{##4##1\ ##2}]{\hspace*{-\labelsep}##4##3\@thmcounterend}##5}
     \def\@Opargbegintheorem##1##2##3##4{##4\trivlist
         \item[\hskip\labelsep{##3##1}]{\hspace*{-\labelsep}##3##2\@thmcounterend}}}{}
%



==> polynomialmaps.tex <==


\section{ Generally neighborly polynomial maps}\label{sec:polymap}
Recall that \cref{prob:dim} asks for the minimal dimension of the ambient space in which a generally $k$-neighborly embedded manifold exists. In this section we study an algebraic version of this problem. Instead of manifolds, we will consider algebraic varieties. And instead of embeddings we consider polynomial maps. 

The problem we study concerns \emph{generally $k$-neighborly polynomial maps}.

\begin{definition}\label{def:generallyneighborly}
Assume $\varphi: \Rl^d \to \Rl^p$ is a polynomial map such that $V:=\varphi(\Rl^d)$ is a $d$-dimensional irreducible real algebraic variety with a smooth real point. Assume also that $\varphi$ is equipped with a general position assumption $G$ for point sets in $\Rl^d$. Then $\varphi$ is a \emph{generally $k$-neighborly polynomial map of $\Rl^d$} if for any finite set $S$ of points in $\Rl^d$ in general position (according to $G$), $\varphi(S)$ is the vertex set of a $k$-neighborly polytope. It is called a \emph{generally neighborly polynomial map of $\Rl^d$} if it is generally $\lfloor\frac{p}{2} \rfloor$-neighborly. 
\end{definition}

The variety $V$ in the above definition is called a \emph{generally $k$-neighborly algebraic variety}. 

Generally $k$-neighborly polynomial maps can be thought of as a special case of generally $k$-neighborly embeddings where we consider polynomial maps rather than arbitrary embeddings. However, they are not strictly speaking a special case because a polynomial map may not be an embedding if it is not injective. However, because we assume that the variety $V$ in the above definition contains a smooth real point, it is necessarily the case that $V$ has real dimension $d$. This is due to the fact that around a smooth point of an $d$-dimensional variety there is a neighborhood homeomorphic to $\Rl^d$ \cite{Bochnak}. Therefore, while generally $k$-neighborly polynomial maps of $\Rl^d$ may not be generally $k$-neighborly embeddings of $\Rl^d$, they are  generally $k$-neighborly embeddings of some open subset of $\Rl^d$.



To be clear, the question we are dealing with in this section is the following. 
\begin{problem}\label{probpoly}
What is the smallest dimension $p:=p_{g,P}(k,d)$ of the image space for which a generally
$k$-neighborly polynomial map $\varphi: \Rl^d \to \Rl^p$ exists? 
\end{problem}


%Assuming that the images of our maps are varieties allow us to use several facts from real algebraic geometry. These facts, which are not true in general for real embedded manifolds, are what allow us to prove \cref{Conjecture:conjecture} in the case of polynomial maps which map $\Rl^d$ into a variety. Most crucially, we use the fact that algebraic varieties can be decomposed into a union of irreducible components.
We will prove the following theorem which completely resolves \cref{probpoly}.

\begin{theorem}\label{prop:lowerbound}
Assume that $\varphi: \Rl^d \to \Rl^p$ is a generally $k$-neighborly polynomial map of $\Rl^d$. 
Then $p \geq 2k+d-1$. Therefore, $p_{g,P}(k,d) \ge  2k+d-1$.
\end{theorem}

\cref{prop:lowerbound} combined with \cref{thm:embedding} show that $p_{g,P}(k,d) = 2k+d-1$. 

Unfortunately, it is not clear how to adapt our proof technique to handle polynomial maps whose image is not a variety. 
As an example, consider the map $HV_{2}^2: \Rl^2 \to \Rl^3$ where $HV_{2}^2(x,y) = (x^2,xy,y^2)$. 
The image of $HV_{2}^2$ is a cone with vertex at the origin which is not a variety. 
%It is \say{half} of the variety $Z(y^2-xz) \subset \Rl^3$ which consists of a double cone with vertex at the origin. 
Despite examples such as this, many interesting examples of generally $k$-neighborly polynomial maps do satisfy the requirement that their image is a variety. Below we list some examples of maps that are either generally neighborly embeddings or generally neighborly polynomial maps, or both.
\begin{example}
The degree 2 Veronese map of the plane is a generally neighborly polynomial map \emph{and} a generally neighborly embedding of $\Rl^2$ into $\Rl^5$. 
\end{example}
\begin{example}
The map $HV_{2m}^2$ is a generally neighborly embedding of the open first quadrant into $\Rl^{2m+1}$.
\end{example}
\begin{example}
The map $\varphi$ from the proof of \cref{thm:embedding} is a generally $k$-neighborly embedding \emph{and} a generally $k$-neighborly polynomial map of $\Rl^d$ into $\Rl^{2k+d-1}$.  
\end{example}
Before proving \cref{prop:lowerbound} we need to establish the connection between generally $k$-neighborly maps and \emph{weakly $k$-neighborly} sets. 

